Inverse Neural Rendering for Explainable Multi-Object Tracking

Today, most methods for image understanding tasks rely on feed-forward neural networks. While this approach has allowed for empirical accuracy, efficiency, and task adaptation via fine-tuning, it also comes with fundamental disadvantages. Existing networks often struggle to generalize across different datasets, even on the same task. By design, these networks ultimately reason about high-dimensional scene features, which are challenging to analyze. This is true especially when attempting to predict 3D information based on 2D images. We propose to recast 3D multi-object tracking from RGB cameras as an \emph{Inverse Rendering (IR)} problem, by optimizing via a differentiable rendering pipeline over the latent space of pre-trained 3D object representations and retrieve the latents that best represent object instances in a given input image. To this end, we optimize an image loss over generative latent spaces that inherently disentangle shape and appearance properties. We investigate not only an alternate take on tracking but our method also enables examining the generated objects, reasoning about failure situations, and resolving ambiguous cases. We validate the generalization and scaling capabilities of our method by learning the generative prior exclusively from synthetic data and assessing camera-based 3D tracking on the nuScenes and Waymo datasets. Both these datasets are completely unseen to our method and do not require fine-tuning. Videos and code are available at https://light.princeton.edu/inverse-rendering-tracking/.

==> definition.tex <==

% formatting stuff

\definecolor{Gray}{rgb}{0.5,0.5,0.5}
\definecolor{darkblue}{rgb}{0,0,0.7}
\definecolor{orange}{rgb}{1,.5,0} % something readable but different from todo
\definecolor{red}{rgb}{1,0,0} % something readable but different from todo

% taken from https://designnavigator.daimler.com/Daimler_Color_System
\definecolor{dai_ligth_grey}{RGB}{230,230,230}
\definecolor{dai_ligth_grey20K}{RGB}{200,200,200}
\definecolor{dai_ligth_grey40K}{RGB}{158,158,158}
\definecolor{dai_ligth_grey60K}{RGB}{112,112,112}
\definecolor{dai_ligth_grey80K}{RGB}{68,68,68}
\definecolor{dai_petrol}{RGB}{0,103,127}
\definecolor{dai_petrol20K}{RGB}{0,86,106}
\definecolor{dai_petrol40K}{RGB}{0,67,85}
\definecolor{dai_petrol80}{RGB}{0,122,147}
\definecolor{dai_petrol60}{RGB}{80,151,171}
\definecolor{dai_petrol40}{RGB}{121,174,191}
\definecolor{dai_petrol20}{RGB}{166,202,216}
\definecolor{dai_deepred}{RGB}{113,24,12}
\definecolor{dai_deepred20K}{RGB}{90,19,10}
\definecolor{dai_deepred40K}{RGB}{68,14,7}
%\definecolor{violettblau}{cmyk}{0.9, 0.6, 0, 0}
\definecolor{rot}{RGB}{238, 28 35}
\definecolor{apfelgruen}{RGB}{140, 198, 62}
%\definecolor{gelb}{RGB}{255, 229, 0}
\definecolor{orange}{RGB}{244, 111, 33}
\definecolor{pink}{RGB}{237, 0, 140}
\definecolor{lila}{RGB}{128, 10, 145}
%\definecolor{hellgrau}{RGB}{224, 224, 224}
%\definecolor{mittelgrau}{RGB}{128, 128, 128}
%\definecolor{dunkelgrau}{RGB}{80,80,80}
\definecolor{anthrazit}{RGB}{19, 31, 31}

\newcommand{\heading}[1]{\noindent\textbf{#1}}
\newcommand{\note}[1]{{\em{\textcolor{orange}{#1}}}}
\newcommand{\todo}[1]{{\textcolor{red}{\bf{TODO: #1}}}}
% \newcommand{\comment}[1]{{\small{\emph{\textcolor{Gray}{#1}}}}}
\newcommand{\comments}[1]{{\em{\textcolor{orange}{#1}}}}
% \newcommand{\changed}[1]{{\textcolor{blue}{#1}}}
\newcommand{\changed}[1]{#1}
\newcommand{\place}[1]{ \begin{itemize}\item\textcolor{darkblue}{#1}\end{itemize}}
\newcommand{\de}{\mathrm{d}}

\newcommand{\normlzd}[1]{{#1}^{\textrm{aligned}}}

% dimensions
\newcommand{\ttime}{\tau}               % time coordinate
\newcommand{\x}{\Vect{x}}               % spatial coordinates in vectorized form
\newcommand{\z}{z}               % depth coordinate of volume

\newcommand{\npixels}{n}               % num pixels
\newcommand{\ntime}{t}               % num timesteps

%image formation
\newcommand{\illfunc}     {g}
\newcommand{\pathfunc}     {s}
\newcommand{\camfunc}     {f}

% notation for image formation
\newcommand{\irradiance}{E}
\newcommand{\exposure}{b}
\newcommand{\pmdfunc}{f}                % modulation on the PMD side
\newcommand{\lightfunc}{g}              % modulation of the light
\newcommand{\period}{T}                 % temporal period of the modulation
\newcommand{\freqm}{\omega}                % frequency of modulation
\newcommand{\illphase}{\rho}             % frequency of modulation harmonics
\newcommand{\sensphase}{\psi}             % frequency of modulation harmonics of pmd camera
\newcommand{\pmdphase}{\phi}            % phase of PMD modulation
\newcommand{\omphi}{{\omega,\phi}}      % shorthand for freq/phase pair
\newcommand{\numperiod}{N}              % #periods integrated over
\newcommand{\att}{\alpha}               % geometric & photometric attenuation
\newcommand{\pathspace}{{\mathcal{P}}}  % space of all light paths

% regular modulation based cameras
\newcommand{\atan}{\operatorname{atan}}

% math stuff
\newcommand{\Fourier}{\mathfrak{{F}}}         % fourier transform
\newcommand{\conv}     {\otimes}
\newcommand{\corr}     {\star}
\newcommand{\Mat}[1]    {{\ensuremath{\mathbf{\uppercase{#1}}}}} %Matrix 
\newcommand{\Vect}[1]   {{\ensuremath{\mathbf{\lowercase{#1}}}}} %Vector
\newcommand{\Id}				{\mathbb{I}} %Identity matrix
\newcommand{\Diag}[1] 	{\operatorname{diag}\left({ #1 }\right)} %Diagonalized matrix
\newcommand{\Opt}[1] 	  {{#1}_{\text{opt}}} %Optimal point of an optimization
\newcommand{\CC}[1]			{{#1}^{*}} %Convex conjugate
\newcommand{\Op}[1]     {\Mat{#1}} %Operator
\newcommand{\minimize}[1] {\underset{{#1}}{\operatorname{argmin}} \: \: } %Minimize w.r.t.
\newcommand{\maximize}[1] {\underset{{#1}}{\operatorname{argmax}} \: \: } %Maximize w.r.t.  
\newcommand{\grad}      {\nabla}

% notation for method
\newcommand{\Basis}{\Mat{H}}         		% Matrix basis
\newcommand{\Corr}{\Mat{C}}             % measurement matrix
\newcommand{\correlem}{\bold{c}}             % measurement matrix element
\newcommand{\meas}{\Vect{b}}            % measurement vector
\newcommand{\Meas}{\Mat{B}}            % measurement matrix
\newcommand{\MeasNormalized}{\Mat{B}^{\textrm{new}}}            % measurement matrix
\newcommand{\Img}{H}                    % transient image
\newcommand{\img}{\Vect{h}}             % vectorized image
\newcommand{\latentresponse}{\alpha}



\newenvironment{customlegend}[1][]{%
        \begingroup
        % inits/clears the lists (which might be populated from previous
        % axes):
        \csname pgfplots@init@cleared@structures\endcsname
        \pgfplotsset{#1}%
    }{%
        % draws the legend:
        \csname pgfplots@createlegend\endcsname
        \endgroup
    }%

    % makes \addlegendimage available (typically only available within an
    % axis environment):
    \def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}


==> main_paper/tables/fig_Waymo_tracking.tex <==
\begin{figure*}[t!]
	\centering
\resizebox{1.\linewidth}{!}{
	\renewcommand{\arraystretch}{0.5}
	\begin{tabular}{@{}c@{\hskip .05cm}c@{\hskip .05cm}c@{\hskip .05cm}c@{\hskip .05cm}c@{\hskip .05cm}c@{}}
		\centering
            &
		{\small Input $t_0$}&
		{\small Tracked $t_0$}&
		{\small Tracked $t_1$}&
		{\small Tracked $t_2$}&
		{\small Tracked $t_3$}\\

            \rotatebox[origin=c]{90}{{\footnotesize	Highway}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene1/waymo_s50_f45.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene1/waymo_s50_f45_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene1/waymo_s50_f46_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene1/waymo_s50_f47_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene1/waymo_s50_f48_bbox.png}}\\[0.9cm]

            \rotatebox[origin=c]{90}{{\footnotesize	Urban}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene2/waymo_44_38_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene2/waymo_44_38_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene2/waymo_44_39_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene2/waymo_44_40_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/waymo_main/scene2/waymo_44_41_bbox.png}}\\%[0.0cm]
		
		
	\end{tabular}
	}
\vspace{-6pt}
\caption{Without changing the model or training on the dataset, our proposed method can generalize well to the Waymo Open Driving Dataset ~\cite{sun2020scalability}. Similar to Fig \ref{fig:nuScenes_results}, from left to right, we show (i) observed images from diverse scenes from the dataset at timestep $k=0$; (ii) an overlay of the closest generated object and predicted 3D bounding boxes at timestep $k=0, 1, 2 \text{ and } 3$. The color of the bounding boxes for each object corresponds to the predicted tracklet ID. Our method does not lose any tracks even on a different unseen dataset in diverse scenes, validating that the approach generalizes.}\label{fig:waymo_results}
% \vspace*{-14pt}
\end{figure*}

% We first show the initial input frame at timestep k=0. Next to it, we present an overlay of the closest generated object and the refined bounding boxes. Reconstructions and bounding boxes for the next 3 frames are presented next to it. \todo{Description. Talk about color coding and that you don't lose any detections.}

==> main_paper/tables/fig_ablate_scheduler.tex <==
% \begin{figure}[t!]
% 	% \vspace{-12pt}
% 	 \renewcommand{\arraystretch}{0.4}
% 	\centering
% 	\resizebox{1\columnwidth}{!}{%
% 	\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
% 	    {\small (a) Input Frame} & {\small (b) w/ Schedule} & {\small (c) wo/ Schedule} \\
%     	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
%     	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
%     	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png}\\
%     	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/gt/82_60_gt_img.png}&
%     	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/sched/82_60_shed.png}&
%     	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/no_sched/82_60_no_shed.png}\\
%     \end{tabular}}\vspace*{-6pt}
% 	\caption{\todo{Make split figure} \textbf{Effect of Optimization Schedule.} (a) observed image, (b) optimized generations using the proposed schedule (see 3.1 \& 3.3), (c) optimized generations using no schedule.
%  % , i.e. such that texture codes, shape codes, rotations, translations, and scales are all simultaneously optimized. The ground truth images are faded to show our rendered objects clearly. 
%     % The bottom row shows images zoomed in to clearly show our rendered objects.
%     % Our schedule allows for more stable optimization, with rendered objects more closely resembling the observed ones. 
%  } 
% 	\label{fig:opt_scheduler}
% 	% \vspace{-8pt}
% \end{figure}


\begin{figure}[t!]
% \vspace{-12pt}
\renewcommand{\arraystretch}{0.4}
\centering
% \resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
    \multicolumn{2}{c}{(a) Input Frame} & \multicolumn{2}{c}{(b) Full (ours)} & \multicolumn{2}{c}{(c) \underline{No Schedule}} \\
    \includegraphics[width=.16\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
    \includegraphics[width=.16\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/gt/82_60_gt_img.png}&
    \includegraphics[width=.16\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
    \includegraphics[width=.16\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/sched/82_60_shed.png}&
    \includegraphics[width=.16\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png}&    	\includegraphics[width=.16\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/no_sched/82_60_no_shed.png}\\
    \end{tabular}
% }
    \vspace*{-6pt}
    \caption{\textbf{Effect of Optimization Schedule.} (a) observed image, (b) optimized generations using the proposed schedule in Sec.~\ref{sec:method}, (c) optimized generations using no schedule. \todo{move into table 2.}
 % , i.e. such that texture codes, shape codes, rotations, translations, and scales are all simultaneously optimized. The ground truth images are faded to show our rendered objects clearly. 
    % The bottom row shows images zoomed in to clearly show our rendered objects.
    % Our schedule allows for more stable optimization, with rendered objects more closely resembling the observed ones. 
} 
	\label{fig:opt_scheduler}
	% \vspace{-8pt}
\end{figure}

==> main_paper/tables/fig_additional_nuscenes_results.tex <==
\newpage
\begin{figure*}[h!]
	\vspace{-5pt}
	\centering
	\resizebox{0.98\linewidth}{!}{
	\renewcommand{\arraystretch}{0.5}
	\begin{tabular}{@{}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{}}
		\centering
            &
		{\huge Input $t_0$}&
		{\huge Tracked $t_0$}&
		{\huge Tracked $t_1$}&
		{\huge Tracked $t_2$}&
		{\huge Tracked $t_3$}\\

            \rotatebox[origin=c]{90}{{\Large	  Crossing 1}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/26_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/26_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/27_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/28_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/29_bbox.png}}\\[1.9cm]
  
		\rotatebox[origin=c]{90}{{\Large	 Traffic}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/23.png}} &
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/24.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/25.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/26.png}}\\[1.9cm]
  
            \rotatebox[origin=c]{90}{{\Large	Urban 1}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/21.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/22.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/23.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/4.png}}\\[1.9cm]
  
            \rotatebox[origin=c]{90}{{\Large	Urban 2}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/2_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/2_out.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/3_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/4_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/5_out.png}}\\[1.9cm]

        \rotatebox[origin=c]{90}{{\Large	 Urban 3}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_0_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_0_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_1_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_2_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_3_bbox.png}}\\[1.9cm]
        
    \rotatebox[origin=c]{90}{{\Large	  Crossing}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_8_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_8_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_9_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_10_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_11_bbox.png}}\\[1.9cm]

    \rotatebox[origin=c]{90}{{\Large	  Crossing 2}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/27.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/28.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/29.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/30.png}}\\[1.9cm]

  \rotatebox[origin=c]{90}{{\Large	  Left View}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/14.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/15.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/16.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/17.png}}\\[1.9cm]

 \rotatebox[origin=c]{90}{{\Large	Parking}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/29.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/30.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/31.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/32.png}}\\[1.9cm]


  \rotatebox[origin=c]{90}{{\Large	  River}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/0_gt_new.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/0_new_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/1_new_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/bbox_2_new.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/bbox_3_new.png}}\\[1.9cm]

	\end{tabular}
	}
	\caption{Additional visualizations on nuScenes~\cite{caesar2020nuscenes}. From left to right, we show (i) observed images from diverse scenes at timestep $k=0$; (ii) an overlay of the optimized generated object and its 3D bounding boxes at timestep $k=0, 1, 2 \text{ and } 3$. The color of the bounding boxes for each object corresponds to the predicted tracklet ID. We see that our method can accurately reconstruct objects in diverse scenarios.}
	\label{fig:additional_nuScenes_results}

\end{figure*}
\newpage

==> main_paper/tables/fig_additional_waymo_results.tex <==
\newpage
\begin{figure*}[ht!]
	\vspace{-5pt}
	\centering
	\resizebox{0.9\linewidth}{!}{
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{@{}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{}}
		\space
            &
		{\huge Input $t_0$}&
		{\huge Tracked $t_0$}&
		{\huge Tracked $t_1$}&
		{\huge Tracked $t_2$}&
		{\huge Tracked $t_3$}\\

            \rotatebox[origin=c]{90}{{\Large	  Residential 1}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/35.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/36.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/37.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/38.png}}\\[2.3cm]

  \rotatebox[origin=c]{90}{{\Large	  Residential 2}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/36.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/37.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/38.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/39.png}}\\[2.3cm]

 \rotatebox[origin=c]{90}{{\Large	  Residential 3}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/2.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/4.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/5.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/6.png}}\\[2.3cm]
   
 \rotatebox[origin=c]{90}{{\Large	  Dense Urban}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/0.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/1.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/2.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/3.png}}\\[2.3cm]
  
		\rotatebox[origin=c]{90}{{\Large	 Suburban 1}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/7.png}} &
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/9.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/10.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/10.png}}\\[2.3cm]
  
            \rotatebox[origin=c]{90}{{\Large	 Suburban 2}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/5.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/6.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/7.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/8.png}}\\[2.3cm]

        \rotatebox[origin=c]{90}{{\Large	  Suburban 3}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/5.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/6.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/7.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/8.png}}\\[2.3cm]
        
        \rotatebox[origin=c]{90}{{\Large	  Suburban 4}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/22.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/23.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/24.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/25.png}}\\[2.3cm]


\rotatebox[origin=c]{90}{{\Large	  Highway}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/5.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/6.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/7.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/8.png}}\\[2.3cm]

  %           \rotatebox[origin=c]{90}{{\Large	Residential 2}}&
  % 		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/gt_img.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/5.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/6.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/7.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/8.png}}\\[2.3cm]


\end{tabular}}
\caption{Additional visualizations on Waymo~\cite{sun2020scalability}. From left to right, we show (i) observed images from diverse scenes at timestep $k=0$; (ii) an overlay of the optimized generated object and its 3D bounding boxes at timestep $k=0, 1, 2 \text{ and } 3$. The color of the bounding boxes for each object corresponds to the predicted tracklet ID. We see that our method can accurately match and track tracklets in diverse scenarios in the Waymo dataset as well, confirming that the method is dataset-agnostic.}
\label{fig:additional_waymo_results}
\end{figure*}
\newpage

==> main_paper/tables/fig_interpretability.tex <==
% \begin{wrapfigure}{r}{0.6\linewidth}
\begin{figure}[bt!]
	\centering
\resizebox{1.\linewidth}{!}{
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{@{}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{}}
		\space
            &
		{\huge Input $t_0$}&
		{\huge Tracked $t_0$}&
		{\huge Tracked $t_1$}&
		% {\small Tracked $t_2$}&
		% {\small Tracked $t_3$}\\

   %           \rotatebox[origin=c]{90}{{\large  Similar colored cars}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/26_gt.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/26_bbox.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/28_bbox.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}\\[0.95cm]

           \rotatebox[origin=c]{90}{{\Large \textbf{(a)} Shadow}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/21.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/22.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
  \\[0.01cm]

            \rotatebox[origin=c]{90}{{\Large \textbf{(b)} Reflection}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/5.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/6.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
  \\[0.01cm]
  
           \rotatebox[origin=c]{90}{{\Large \textbf{(c)} Occlusion}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene7/0118_4_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene7/0118_4_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene7/0118_6_bbox.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
   \\[0.01cm]
        
        \rotatebox[origin=c]{90}{{\Large \textbf{(d)} Obstruction}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/rainy_scene/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/rainy_scene/30.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/rainy_scene/31.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
   \\[0.01cm]

   		\rotatebox[origin=c]{90}{{\Large \textbf{(e)} Det. Accuracy}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene2/2_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene2/2)bbix.png}} &
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene2/3_bbox.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
\end{tabular}}
\caption{Examples of failure cases, such as lighting (shadows and reflections) or occluded objects, where the reconstructed object differs significantly from the observed object. These visualizations allow us to understand exactly why our model fails at reconstructing and tracking objects. This also allows us to identify ways the representation model and perception pipeline can be improved to incorporate effects that cause the method to fail.}
	\label{fig:interpretability}
 \end{figure}
% \end{wrapfigure}


==> main_paper/tables/fig_nuScenes_3D_BEV.tex <==
\begin{figure}[t!]
	% \vspace{-12pt}
	 \renewcommand{\arraystretch}{0.4}
	\centering
	\resizebox{1\columnwidth}{!}{%
	\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
 
    \multicolumn{1}{c}{\large (i) Input Frame} & \multicolumn{1}{c}{\large (ii) INR 3D Generation} & \multicolumn{1}{c}{\large (iii) INR BEV Layout} \\
     
    \includegraphics[width=.5\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/BEV_and_3D/scene1/nusc_sc_3_cam_5_f9_gt.png}&

    \includegraphics[width=.5\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/BEV_and_3D/scene1/sc_3_cam5_f9_rgb_out.png}&

    \includegraphics[width=.5\columnwidth, trim={2.1cm 2cm 1.9cm 2cm},clip]{fig/BEV_and_3D/BEV_axis_1.png}\\

    \includegraphics[width=.5\columnwidth, trim={26cm 6.7cm 12.5cm 15cm},clip]{fig/BEV_and_3D/scene2/gt_img.png}&
    \includegraphics[width=.5\columnwidth, trim={26cm 6.7cm 12.5cm 15cm},clip]{fig/BEV_and_3D/scene2/rgb_out.png}&
    \includegraphics[width=.5\columnwidth, trim={2.1cm 2cm 1.9cm 2cm},clip]{fig/BEV_and_3D/BEV_axis_2.png}\\
     
    % \textbf{\large (a)} & \textbf{\large (b)} & \textbf{\large (a)} & \textbf{\large (b)} & \textbf{\large (a)} & \textbf{\large (b)} \\
    \end{tabular}}
    % \vspace*{-6pt}
\caption{\textbf{Layout Generation Through Inverse Rendering.} From left to right, we show (i) observed image from a single camera for two scenes, (ii) test-time optimized inverse rendered (IR) objects of class ``car'', and (iii) Bird's Eye View (BEV) layout of the scene. In the BEV layout, black boxes represent ground truth, and the colored boxes represent predicted BEV boxes. The bottom shows a zoomed-in region at a 60 m distance (see BEV layout). Even in this setting, our method recovers the coarse appearance, shape of the objects, pose, and size,} 
\label{fig:BEV3D_fig}
% \vspace*{-16pt}
\end{figure}



==> main_paper/tables/fig_nuScenes_tracking.tex <==
% \begin{figure*}[t!]
% 	% \vspace{-20pt}
% 	\centering
% 	\resizebox{0.98\linewidth}{!}{
% 	\renewcommand{\arraystretch}{0.5}
% 	\begin{tabular}{@{}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{}}
% 		\centering
%             &
% 		{\small Input $t_0$}&
% 		{\small Tracked $t_0$}&
% 		{\small Tracked $t_1$}&
% 		{\small Tracked $t_2$}&
% 		{\small Tracked $t_3$}\\

%             \rotatebox[origin=c]{90}{{\footnotesize	  Suburban}}&
% 		 \raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_2_gt.png}}&
% 		 \raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_2_bbox.png}}&
% 		 \raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_3_bbox.png}}&
% 		 \raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_4_bbox.png}}&
% 		 \raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_5_bbox.png}}\\[0.95cm]
  
% 		\rotatebox[origin=c]{90}{{\footnotesize	 Dense Urban}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_30_gt.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_30_bbox.png}} &
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_31_bbox.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_32_bbox.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_33_bbox.png}}\\[0.7cm]
  
%             \rotatebox[origin=c]{90}{{\footnotesize	 Clutter}}&
%   		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/28_gt_img.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/35_28_bbox.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/35_29_bbox.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/35_30_bbox.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/35_31_bbox.png}}\\[0.7cm]
  
%             \rotatebox[origin=c]{90}{{\footnotesize	Parking lot}}&
%   		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/gt_2.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/bbox_0.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/bbox_1.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/bbox_3.png}}&
% 		\raisebox{-0.5\height}{\includegraphics[width=.19\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/bbox_33.png}}\\%[0.95cm]
		
% 	\end{tabular}
% }
% 	\vspace{-6pt}
% 	\caption{Tracking via Inverse Neural Rendering on nuScenes~\cite{caesar2020nuscenes}. From left to right, we show (i) observed images from diverse scenes at timestep $k=0$; (ii) an overlay of the optimized generated object and its 3D bounding boxes at timestep $k=0, 1, 2 \text{ and } 3$. The color of the bounding boxes for each object corresponds to the predicted tracklet ID. We see that even in such diverse scenarios, our method does not lose any tracks and performs robustly across all scenarios, although the dataset is unseen.}
% 	\label{fig:nuScenes_results}
%  	\vspace{-12pt}
% \end{figure*}

\begin{figure*}[t!]
	% \vspace{-20pt}
	\centering
	\resizebox{1.\linewidth}{!}{
	\renewcommand{\arraystretch}{0.5}
	\begin{tabular}{@{}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{}}
		\centering
            &
		{\small Input $t_0$}&
		{\small Tracked $t_0$}&
		{\small Tracked $t_1$}&
		{\small Tracked $t_2$}&
		{\small Tracked $t_3$}\\

            \rotatebox[origin=c]{90}{{\footnotesize	  Suburban}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_2_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_2_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_3_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_4_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene2/0484_5_bbox.png}}\\[0.75cm]
  
		\rotatebox[origin=c]{90}{{\footnotesize	 Urban}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_30_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_30_bbox.png}} &
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_31_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_32_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene3/0496_33_bbox.png}}\\[0.75cm]
  
            \rotatebox[origin=c]{90}{{\footnotesize	 Clutter}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/28_gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/35_28_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/35_29_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/35_30_bbox.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene6/35_31_bbox.png}}\\[0.75cm]
  
            \rotatebox[origin=c]{90}{{\footnotesize	Parking lot}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/gt_2.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/bbox_0.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/bbox_1.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/bbox_3.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.32\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/nuScenes_main/scene7/bbox_33.png}}\\%[0.95cm]
		
	\end{tabular}
	}
\vspace*{-6pt}
\caption{Tracking via Inverse Neural Rendering on nuScenes~\cite{caesar2020nuscenes}. From left to right, we show (i) observed images from diverse scenes at timestep $k=0$; (ii) an overlay of the optimized generated object and its 3D bounding boxes at timestep $k=0, 1, 2 \text{ and } 3$. The color of the bounding boxes for each object corresponds to the predicted tracklet ID. We see that even in such diverse scenarios, our method does not lose any tracks and performs robustly across all scenarios, although the dataset is unseen.}\label{fig:nuScenes_results}
\vspace*{-12pt}
\end{figure*}

==> main_paper/tables/fig_optimization.tex <==
\begin{figure*}[t!]
	% \vspace{-12pt}
	% \renewcommand{\arraystretch}{0.5}
\centering
\resizebox{1.\linewidth}{!}{%
\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}

{Input Frame} & {Initial Guess} & {Texture Fitting} & {Object Pose Fitting} & {Shape Fitting} \\
	    
\includegraphics[width=.5\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optim/optim_input.png}&
\includegraphics[width=.5\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optim/init_im_w_bbox.png}&
\includegraphics[width=.5\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optim/texture_im_w_bbox.png}&
\includegraphics[width=.5\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optim/pose_im_pil.png}&
\includegraphics[width=.5\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optim/final_im_w_bbox.png}\\
& \multicolumn{4}{r}{\textit{Input frame is faded for visibility.}} \\
\end{tabular}}
\vspace*{-6pt} 
\caption{\textbf{Optimization Process.} From left to right, we show (i) the observed image, (ii) the rendering predicted by the initial starting point latent embeddings, 
(iii) the predicted rendered objects after the texture code is optimized (iv) the predicted rendered objects after the translation, scale, and rotation are optimized, and (v) the predicted rendered objects after the shape latent code is optimized. The ground truth images are faded to show our rendered objects clearly. Our method is capable of refining the predicted texture, pose, and shape over several optimization steps, even if initialized with poses or appearance far from the target -- all corrected through inverse rendering.} 
\label{fig:optim}
% \vspace*{-16pt}
\end{figure*}


==> main_paper/tables/fig_optimization_no_embedding.tex <==
\begin{figure}[t!]
	\centering
\resizebox{0.9\linewidth}{!}{
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{@{}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{}}
		{ Input}&
		{w/o $\mathcal{L}_{embed}$}&
		{w/ $\mathcal{L}_{embed}$}&
	
\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optimization_no_trunc_reg/scene2/gt_img.png}&
\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optimization_no_trunc_reg/scene2/noembed.png}&
\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optimization_no_trunc_reg/scene2/im_w_bbox_rgb_out.png}
\end{tabular}}
\caption{\textbf{Truncation Trick.} From left to right, (i) The input observed image, (ii) results without truncation regularize applied and (iii) results with a truncation regularize applied. For images (ii) and (iii), we also show bounding boxes for each object color-coded by the respective predicted object IDs. As shown here, applying the truncation regularizer helps us achieve more accurate textures and better shapes and colors for the predicted car surface by forcing the optimized embedding to be ``well behaved'', i.e., close to the distribution of latent embeddings seen during the training by our representation model.}
\label{fig:optimization_truncation}
\end{figure}




==> main_paper/tables/rebuttal_fig_optimization_supplement_no_scehdule.tex <==
\begin{figure}[ht!]
	% \vspace{-12pt}
	 \renewcommand{\arraystretch}{0.4}
	\centering
	\resizebox{1\columnwidth}{!}{%
	\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
	    {\small (a) Input Frame} & {\small (b) w/ Schedule} & {\small (c) wo/ Schedule} \\
    	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
    	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
    	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png}\\
    	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/gt/82_60_gt_img.png}&
    	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/sched/82_60_shed.png}&
    	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/no_sched/82_60_no_shed.png}\\
    \end{tabular}}\vspace*{-6pt}
	\caption{\textbf{Effect of Optimization Schedule.} (a) observed image, (b) optimized generations using the proposed schedule (see 3.1 \& 3.3), (c) optimized generations using no schedule.
 % , i.e. such that texture codes, shape codes, rotations, translations, and scales are all simultaneously optimized. The ground truth images are faded to show our rendered objects clearly. 
    % The bottom row shows images zoomed in to clearly show our rendered objects.
    % Our schedule allows for more stable optimization, with rendered objects more closely resembling the observed ones. 
 } 
	\label{fig:opt_rebuttal}
	\vspace{-8pt}
\end{figure}

% \begin{figure}[t!]
%     % \vspace{-12pt}
%     \renewcommand{\arraystretch}{0.4}
%     \centering
%     \resizebox{1\columnwidth}{!}{%
%     \begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
%         {\small Input Frame} & {\small Initial Guess} & {\small w/ schedule} & {\small wo/ schedule} \\
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/init_guess/11_102_init.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png}\\
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}\\
%     \end{tabular}}\vspace*{-6pt}
%     \caption{\textbf{Effect of having an optimization schedule.} From left to right, we show (i) observed image from a single camera, (ii) initial guess, (iii) with schedule, and (iv) without schedule. \todo{describe the figure.}} 
%     \label{fig:opt_supplement}
%     \vspace{-8pt}
% \end{figure}


==> main_paper/tables/rebuttal_matching_ablations.tex <==
\begin{table}[t!]\label{tab:ablations}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|lll}
\hline
\hline
    Method (split)            & AMOTA $\uparrow$  & Recall $\uparrow$ & MOTA $\uparrow$   \\
    \hline
    AB3DMOT + CP (test) & 0.387             & 0.506             & 0.284             \\
    \hline
    Best Hyper-parameters (test)       & \textbf{0.402}    & \textbf{0.511}    & \textbf{0.320        }     \\
    \hline
    $w_{iou} = 1.4 $ (validation)   & 0.403             & 0.540             & 0.322               \\
    $w_{center} = 0.9$ (validation) & 0.417             & 0.514             & 0.332             \\
    $w_{embedd} = 0.4$ (validation) & 0.418             & 0.558             & 0.332             \\
    $\tau_{det} = 0.4$ (validation) & 0.397             & 0.567            & 0.326             \\
\hline
\hline
\end{tabular}
}
\caption{\textbf{Optimized Matching and Detection Confidence.} Parameters were optimized on the nuScenes \cite{caesar2020nuscenes} validation set. On the test split our best setting with $w_{iou} = 1.4$, $w_{center} = 0.9$, $w_{embbed} = 0.4$, $\tau_{det} = 0.4$ surpasses the performance of AB3DMOT \cite{weng2020AB3DMOT}, the only baseline not trained on the dataset. Results for other baselines are given in Tab. \ref{tab:nuScenes_results}. }\label{tab:rebuttal_ablations}
\vspace{-12pt}
\end{table}

% 1. AB3DMOT
% 2. $w_{iou} = ...$ ..., ...
% 3. $w_{center}$
% 4. $w_{embedd}$
% 5. $\tau_{det}$
% 6. Best

 




==> main_paper/tables/result_MOT_nuscenes.tex <==
\begin{table*}[t!]
\centering
\vspace*{-8pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|cccc|c}
    \hline \hline
    \textbf{Training} & \textbf{Method} & \textbf{AMOTA} $\uparrow$ &	\textbf{AMOTP} (m) $\downarrow$ &	\textbf{Recall} $\uparrow$ & \textbf{MOTA} $\uparrow$ & \textbf{Modality} \\ 
    \textbf{Data Unseen} &  & &	& & & \\ 
        \hline
%%%%%%%%%%%%%%%% Table Content below
$\times$ & PF-Track~\cite{pang2023PFtrack} & 0.622 & 0.916 & 0.719 & 0.558 & Camera \\
$\times$ & QTrack ~\cite{yang2022qtrack} &  0.692 &  0.753 &  0.760 &  0.596 & Camera \\
$\times$ & QD-3DT ~\cite{hu2021QD3DT} & 0.425 &1.258 &  0.563 &  0.358 & Camera \\
\hline \hline
\textbf{\checkmark} & QD-3DT ~\cite{hu2021QD3DT} (trained on WOD) & 0.000 & 1.893 &  0.226 &  0.000 & Camera \\
$\times$ (CP) & CenterTrack~\cite{zhou2020CenterTrack} & 0.202 &1.195 &0.313 &0.134 & Camera \\
\textbf{\checkmark} (CP) & AB3DMOT ~\cite{weng2020AB3DMOT} & \underline{0.387} & \textbf{1.158} & \underline{0.506} & \underline{0.284} & Camera \\
\textbf{\checkmark} (CP) & Inverse Neural Rendering (ours) & \textbf{0.413} &  \underline{1.189} & \textbf{0.536} & \textbf{0.321} & Camera \\ % updated results as of Feb 15 2024

%%%%%%%%%%%%%%%% Table Content below
\hline \hline
\end{tabular}
}
\caption{\textbf{Quantitative Evaluation for Camera-only Multi-Object Tracking}. Quantitative results on ``cars'' in the test split of the nuScenes tracking dataset~\cite{caesar2020nuscenes}. Our IR-based tracker outperforms AB3DMOT~\cite{weng2020AB3DMOT} on all metrics and CenterTrack~\cite{zhou2020CenterTrack} on accuracy. All three methods use the same detection backbone for fair comparison, while only CenterTrack requires end-to-end training on the dataset.
Additional results show on-par performance of our method with QD-3DT~\cite{hu2021QD3DT} trained on nuScenes \cite{caesar2020nuscenes}. QD-3DT trained on the Waymo Open Dataset (WOD) does not generalize to nuScenes and does not achieve competitive results. Only very recent transformer-based methods, such as PF-Track~\cite{pang2023PFtrack} and the metric learning approach of Q-Track~\cite{yang2022qtrack} achieve a higher score. However, these methods require end-to-end training on each dataset. ``CP'' denotes here the vision-only version of CenterPoint~\cite{zhou2019CenterPointVision} was used for object detection. \textbf{Bold} denotes best and \underline{underlined} second best for methods that did not train on the dataset or use the same detection backbone.}
\label{tab:nuScenes_results}
% \vspace*{-14pt}
\end{table*}

% results without hyper-param tuning
% Inverse Neural Rendering (ours) + CP~\cite{zhou2019CenterPointVision} & Camera& 0.248 &  1.140 & 0.485 & 0.193 & \checkmark \\

% best so far
% AMOTA	AMOTP	RECALL	MOTAR	GT	   MOTA	  MOTP	MT	 ML	  FAF	TP	   FP	 FN	    IDS	    FRAG	TID	    LGD
% 0.402	1.222	0.511	0.651	68518. 0.320  0.627	1281 2096 201.3	33691  11762 33509	1318	1307	1.29	2.30



%     \hline \hline
%     Method & AMOTA $\uparrow$ &	AMOTP (m) $\uparrow$ &	RECALL $\downarrow$ & MOTA $\uparrow$ &   IDS 	$\downarrow$ & No Dataset Training \\
%      &  &	 & & & & Training \\ \hline
% %%%%%%%%%%%%%%%% Table Content below
% PF-Track~\cite{pang2023PFtrack} & 0.622 & 0.916 & 0.719 & 0.558 &  99 &  $\times$ \\
% QTrack ~\cite{yang2022qtrack} &  0.692 &  0.753 &  0.760 &  0.596 & 617 &  $\times$ \\
% QD-3DT ~\cite{hu2021QD3DT}&  0.425 &1.258 &  0.563 &  0.358 &4293 &   $\times$ \\
% CenterTrack (Vision ~\cite{zhou2019CenterPointVision})  &0.202 &1.195 &0.313 &0.134 &2712 &  $\times$ \\
% \hline
% AB3DMOT + ~\cite{zhou2019CenterPointVision} & 0.387 & 1.158 & 0.506 & 0.284 &  1364 & \checkmark  \\
% InverseRenderTrack + ~\cite{zhou2019CenterPointVision} & 0.248 &  1.140 & 0.485 & 0.193 & 2153 & \checkmark \\
% %%%%%%%%%%%%%%%% Table Content below
% \hline \hline



==> main_paper/tables/tab_ablate_matching.tex <==
\begin{table}[ht!]
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|lll}
\hline
\hline
    Method (split)            & AMOTA $\uparrow$  & Recall $\uparrow$ & MOTA $\uparrow$   \\
    \hline
    AB3DMOT + CP (test) & 0.387             & 0.506             & 0.284             \\
    \hline
    Best Hyper-parameters (test)       & \textbf{0.402}    & \textbf{0.511}    & \textbf{0.320        }     \\
    \hline
    $w_{iou} = 1.4 $ (validation)   & 0.403             & 0.540             & 0.322               \\
    $w_{center} = 0.9$ (validation) & 0.417             & 0.514             & 0.332             \\
    $w_{embedd} = 0.4$ (validation) & 0.418             & 0.558             & 0.332             \\
    $\tau_{det} = 0.4$ (validation) & 0.397             & 0.567            & 0.326             \\
\hline
\hline
\end{tabular}
}
\caption{\textbf{Optimized Matching and Detection Confidence.} Parameters were optimized on the nuScenes \cite{caesar2020nuscenes} validation set. On the test split our best setting with $w_{iou} = 1.4$, $w_{center} = 0.9$, $w_{embbed} = 0.4$, $\tau_{det} = 0.4$ surpasses the performance of AB3DMOT \cite{weng2020AB3DMOT}, the only baseline not trained on the dataset. Results for other baselines are given in Tab. \ref{tab:nuScenes_results}. \todo{rewrite} }\label{tab:matching_ablations}
\vspace{-12pt}
\end{table}

==> main_paper/tables/tab_ablate_optim.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|lll}
    \hline
    \hline
    Method & AMOTA $\uparrow$ & Recall $\uparrow$  & MOTA$\uparrow$  \\
    \hline
    No Schedule & 0.102 & 0.224 & 0.110  \\
    \hline
    $\mathcal{L}_{RGB}$ - Eq.~\ref{eq:loss_mse} & N/A  & N/A & N/A  \\
    $\mathcal{L}_{perceptual}$ - Eq.~\ref{eq:loss_lpips} & 0.100 & 0.251 & 0.101 \\
    $\mathcal{L}_{IR}$ - Eq.\ref{eq:loss_mse_lpips}  & 0.103 & 0.236   & 0.112 \\
    $\mathcal{L}_{IR}$ \& $\mathcal{L}_{embed}$ - Eq.\ref{eq:regularize}  & \textbf{0.112} & \textbf{0.264 } & \textbf{0.113} \\
\hline
\hline
\end{tabular}
}
\caption{\todo{(a) Make split figure} \textbf{Ablation Experiments on Optimization Schedule and Loss Components.} Ablations were run on a small subset of the nuScenes~\cite{caesar2020nuscenes} validation set.  $\mathcal{L}_{RGB}$ fails due to the optimizer fitting objects to the background instead, increasing the size of each object resulting in out of memory.}
\label{tab:optim_ablations}
\end{table}


==> main_paper/tables/tab_super_ablations.tex <==
% \input{tables/tab_ablate_matching}
% \input{tables/tab_ablate_optim}
\begin{table}[t]
\caption{\textbf{Ablation Experiments.}}

% 1. Table
\begin{subtable}[t]{1.\linewidth}
\centering
% \vspace*{-8pt}
\renewcommand{\arraystretch}{1.0}
\centering
\resizebox{1.\textwidth}{!}{
\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}

    \multicolumn{1}{c}{(a) Input Frame} &
    \multicolumn{1}{c}{(b) Full (ours)} & 
    \multicolumn{1}{c}{(c) \underline{No Schedule}} \\
    
    \includegraphics[width=.3\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
    \includegraphics[width=.3\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
    \includegraphics[width=.3\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png} \\
    
    \includegraphics[width=.3\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/gt/82_60_gt_img.png} &
    \includegraphics[width=.3\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/sched/82_60_shed.png} &
    \includegraphics[width=.3\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/no_sched/82_60_no_shed.png}\\
    \multicolumn{3}{r}{\textit{Input frame is faded for visibility.}}
    \end{tabular}
}

\caption{\textbf{Effect of Optimization Schedule.} (a) observed image, (b) optimized generations using the proposed schedule in Sec.~\ref{sec:method}, (c) optimized generations using no schedule. This supports the quantitative to the left.}
\label{fig:opt_scheduler}
\end{subtable}
\vspace*{6pt}
% \hfill

% 2. Table
\begin{subtable}[t]{1.\linewidth}
\centering
% \vspace*{-8pt}
\resizebox{1.\textwidth}{!}{
\begin{tabular}{l|lll}
    \hline
    \hline
    Method & AMOTA $\uparrow$ & Recall $\uparrow$  & MOTA$\uparrow$  \\
    \hline
    $\mathcal{L}_{IR}$ \& $\mathcal{L}_{embed}$ - Eq.\ref{eq:regularize}  & \textbf{0.112} & \textbf{0.264 } & \textbf{0.113} \\
    $\mathcal{L}_{IR}$ - Eq.\ref{eq:loss_mse_lpips}  & 0.103 & 0.236   & 0.112 \\
    $\mathcal{L}_{perceptual}$ - Eq.~\ref{eq:loss_lpips} & 0.100 & 0.251 & 0.101 \\
    $\mathcal{L}_{RGB}$ - Eq.~\ref{eq:loss_mse} & N/A  & N/A & N/A  \\
    \hline
    \underline{No Schedule} & 0.102 & 0.224 & 0.110  \\
\hline
\hline
\end{tabular}
}
\caption{\textbf{Optimization Schedule and Loss Components.} Ablations were run on a small subset of the nuScenes~\cite{caesar2020nuscenes} validation set.  $\mathcal{L}_{RGB}$ fails due to the optimizer fitting objects to the background instead, increasing the size of each object resulting in out of memory.}
\label{tab:optim_ablations}
\end{subtable}
\end{table}



% % \input{tables/tab_ablate_matching}
% % \input{tables/tab_ablate_optim}
% \begin{table}[t]
% % 1. Table
% \caption{\textbf{Ablation Experiments}}
% \vspace*{-12pt}
% \begin{subtable}[t]{0.485\linewidth}
% \centering
% \caption{\textbf{Optimization Schedule and Loss Components.} Ablations were run on a small subset of the nuScenes~\cite{caesar2020nuscenes} validation set.  $\mathcal{L}_{RGB}$ fails due to the optimizer fitting objects to the background instead, increasing the size of each object resulting in out of memory.}
% \vspace*{-6pt}
% \resizebox{0.98\textwidth}{!}{
% \begin{tabular}{l|lll}
%     \hline
%     \hline
%     Method & AMOTA $\uparrow$ & Recall $\uparrow$  & MOTA$\uparrow$  \\
%     \hline
%     $\mathcal{L}_{IR}$ \& $\mathcal{L}_{embed}$ - Eq.\ref{eq:regularize}  & \textbf{0.112} & \textbf{0.264 } & \textbf{0.113} \\
%     $\mathcal{L}_{IR}$ - Eq.\ref{eq:loss_mse_lpips}  & 0.103 & 0.236   & 0.112 \\
%     $\mathcal{L}_{perceptual}$ - Eq.~\ref{eq:loss_lpips} & 0.100 & 0.251 & 0.101 \\
%     $\mathcal{L}_{RGB}$ - Eq.~\ref{eq:loss_mse} & N/A  & N/A & N/A  \\
%     \hline
%     \underline{No Schedule} & 0.102 & 0.224 & 0.110  \\
% \hline
% \hline
% \end{tabular}
% }
% \label{tab:optim_ablations}
% \end{subtable}
% \hfill
% % 2. Table
% \begin{subtable}[t]{0.485\linewidth}
% \centering
% \caption{\textbf{Tracking Matching and Detection Confidence.} Parameters were optimized on the nuScenes \cite{caesar2020nuscenes} validation set. On the test split our best setting for $w_{iou}$, $w_{center}$, $w_{embbed}$, $\tau_{det}$ surpasses the performance of AB3DMOT \cite{weng2020AB3DMOT}, the only baseline not trained on the dataset. \todo{exchange with Figure 6}}
% \vspace*{-6pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|lll}
%     \hline
%     \hline
%     Method (split) & AMOTA $\uparrow$ & Recall $\uparrow$ & MOTA $\uparrow$   \\
%     \hline
%     AB3DMOT + CP (test) & 0.387 & 0.506 & 0.284 \\
%     \hline
%     Best Hyper-param. (test) & \textbf{0.402} & \textbf{0.511} & \textbf{0.320} \\
%     \hline
%     $w_{iou} = 1.4 $ (val)   & 0.403             & 0.540             & 0.322 \\
%     $w_{center} = 0.9$ (val) & 0.417             & 0.514             & 0.332 \\
%     $w_{embedd} = 0.4$ (val) & 0.418             & 0.558             & 0.332 \\
%     $\tau_{det} = 0.4$ (val) & 0.397             & 0.567            & 0.326  \\
%     \hline
%     \hline
% \end{tabular}
% }
% \label{fig:matching_ablations}
% \end{subtable}
% \vspace*{-6pt}
% \end{table}

==> tables/fig_ablate_scheduler.tex <==
% \begin{figure}[t!]
% 	% \vspace{-12pt}
% 	 \renewcommand{\arraystretch}{0.4}
% 	\centering
% 	\resizebox{1\columnwidth}{!}{%
% 	\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
% 	    {\small (a) Input Frame} & {\small (b) w/ Schedule} & {\small (c) wo/ Schedule} \\
%     	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
%     	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
%     	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png}\\
%     	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/gt/82_60_gt_img.png}&
%     	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/sched/82_60_shed.png}&
%     	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/no_sched/82_60_no_shed.png}\\
%     \end{tabular}}\vspace*{-6pt}
% 	\caption{\todo{Make split figure} \textbf{Effect of Optimization Schedule.} (a) observed image, (b) optimized generations using the proposed schedule (see 3.1 \& 3.3), (c) optimized generations using no schedule.
%  % , i.e. such that texture codes, shape codes, rotations, translations, and scales are all simultaneously optimized. The ground truth images are faded to show our rendered objects clearly. 
%     % The bottom row shows images zoomed in to clearly show our rendered objects.
%     % Our schedule allows for more stable optimization, with rendered objects more closely resembling the observed ones. 
%  } 
% 	\label{fig:opt_scheduler}
% 	% \vspace{-8pt}
% \end{figure}


\begin{figure}[t!]
% \vspace{-12pt}
\renewcommand{\arraystretch}{0.4}
\centering
% \resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
    \multicolumn{2}{c}{(a) Input Frame} & \multicolumn{2}{c}{(b) Full (ours)} & \multicolumn{2}{c}{(c) \underline{No Schedule}} \\
    \includegraphics[width=.16\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
    \includegraphics[width=.16\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/gt/82_60_gt_img.png}&
    \includegraphics[width=.16\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
    \includegraphics[width=.16\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/sched/82_60_shed.png}&
    \includegraphics[width=.16\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png}&    	\includegraphics[width=.16\columnwidth, trim={22cm 16.68cm 30cm 18cm},clip]{fig/rebuttal_optimization/no_sched/82_60_no_shed.png}\\
    \end{tabular}
% }
    \vspace*{-6pt}
    \caption{\textbf{Effect of Optimization Schedule.} (a) observed image, (b) optimized generations using the proposed schedule in Sec.~\ref{sec:method}, (c) optimized generations using no schedule. \todo{move into table 2.}
 % , i.e. such that texture codes, shape codes, rotations, translations, and scales are all simultaneously optimized. The ground truth images are faded to show our rendered objects clearly. 
    % The bottom row shows images zoomed in to clearly show our rendered objects.
    % Our schedule allows for more stable optimization, with rendered objects more closely resembling the observed ones. 
} 
	\label{fig:opt_scheduler}
	% \vspace{-8pt}
\end{figure}

==> tables/fig_additional_nuscenes_results.tex <==
\newpage
\begin{figure*}[h!]
	\vspace{-5pt}
	\centering
	\resizebox{0.98\linewidth}{!}{
	\renewcommand{\arraystretch}{0.5}
	\begin{tabular}{@{}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{}}
		\centering
            &
		{\huge Input $t_0$}&
		{\huge Tracked $t_0$}&
		{\huge Tracked $t_1$}&
		{\huge Tracked $t_2$}&
		{\huge Tracked $t_3$}\\

            \rotatebox[origin=c]{90}{{\Large	  Crossing 1}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/26_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/26_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/27_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/28_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/29_bbox.png}}\\[1.9cm]
  
		\rotatebox[origin=c]{90}{{\Large	 Traffic}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/23.png}} &
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/24.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/25.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene13/26.png}}\\[1.9cm]
  
            \rotatebox[origin=c]{90}{{\Large	Urban 1}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/21.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/22.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/23.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/4.png}}\\[1.9cm]
  
            \rotatebox[origin=c]{90}{{\Large	Urban 2}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/2_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/2_out.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/3_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/4_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene4/5_out.png}}\\[1.9cm]

        \rotatebox[origin=c]{90}{{\Large	 Urban 3}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_0_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_0_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_1_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_2_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene5/0783_3_bbox.png}}\\[1.9cm]
        
    \rotatebox[origin=c]{90}{{\Large	  Crossing}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_8_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_8_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_9_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_10_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene6/0104_11_bbox.png}}\\[1.9cm]

    \rotatebox[origin=c]{90}{{\Large	  Crossing 2}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/27.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/28.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/29.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene11/30.png}}\\[1.9cm]

  \rotatebox[origin=c]{90}{{\Large	  Left View}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/14.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/15.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/16.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene9/17.png}}\\[1.9cm]

 \rotatebox[origin=c]{90}{{\Large	Parking}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/29.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/30.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/31.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene10/32.png}}\\[1.9cm]


  \rotatebox[origin=c]{90}{{\Large	  River}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/0_gt_new.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/0_new_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/1_new_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/bbox_2_new.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene8/bbox_3_new.png}}\\[1.9cm]

	\end{tabular}
	}
	\caption{Additional visualizations on nuScenes~\cite{caesar2020nuscenes}. From left to right, we show (i) observed images from diverse scenes at timestep $k=0$; (ii) an overlay of the optimized generated object and its 3D bounding boxes at timestep $k=0, 1, 2 \text{ and } 3$. The color of the bounding boxes for each object corresponds to the predicted tracklet ID. We see that our method can accurately reconstruct objects in diverse scenarios.}
	\label{fig:additional_nuScenes_results}

\end{figure*}
\newpage

==> tables/fig_additional_waymo_results.tex <==
\newpage
\begin{figure*}[ht!]
	\vspace{-5pt}
	\centering
	\resizebox{0.9\linewidth}{!}{
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{@{}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{}}
		\space
            &
		{\huge Input $t_0$}&
		{\huge Tracked $t_0$}&
		{\huge Tracked $t_1$}&
		{\huge Tracked $t_2$}&
		{\huge Tracked $t_3$}\\

            \rotatebox[origin=c]{90}{{\Large	  Residential 1}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/35.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/36.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/37.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene1/38.png}}\\[2.3cm]

  \rotatebox[origin=c]{90}{{\Large	  Residential 2}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/36.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/37.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/38.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene9/39.png}}\\[2.3cm]

 \rotatebox[origin=c]{90}{{\Large	  Residential 3}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/2.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/4.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/5.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene10/6.png}}\\[2.3cm]
   
 \rotatebox[origin=c]{90}{{\Large	  Dense Urban}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/0.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/1.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/2.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene11/3.png}}\\[2.3cm]
  
		\rotatebox[origin=c]{90}{{\Large	 Suburban 1}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/7.png}} &
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/9.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/10.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene2/10.png}}\\[2.3cm]
  
            \rotatebox[origin=c]{90}{{\Large	 Suburban 2}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/5.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/6.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/7.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene3/8.png}}\\[2.3cm]

        \rotatebox[origin=c]{90}{{\Large	  Suburban 3}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/5.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/6.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/7.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene5/8.png}}\\[2.3cm]
        
        \rotatebox[origin=c]{90}{{\Large	  Suburban 4}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/22.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/23.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/24.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene6/25.png}}\\[2.3cm]


\rotatebox[origin=c]{90}{{\Large	  Highway}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/5.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/6.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/7.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene8/8.png}}\\[2.3cm]

  %           \rotatebox[origin=c]{90}{{\Large	Residential 2}}&
  % 		\raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/gt_img.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/5.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/6.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/7.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/8.png}}\\[2.3cm]


\end{tabular}}
\caption{Additional visualizations on Waymo~\cite{sun2020scalability}. From left to right, we show (i) observed images from diverse scenes at timestep $k=0$; (ii) an overlay of the optimized generated object and its 3D bounding boxes at timestep $k=0, 1, 2 \text{ and } 3$. The color of the bounding boxes for each object corresponds to the predicted tracklet ID. We see that our method can accurately match and track tracklets in diverse scenarios in the Waymo dataset as well, confirming that the method is dataset-agnostic.}
\label{fig:additional_waymo_results}
\end{figure*}
\newpage

==> tables/fig_interpretability.tex <==
% \begin{wrapfigure}{r}{0.6\linewidth}
\begin{figure}[bt!]
	\centering
\resizebox{1.\linewidth}{!}{
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{@{}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{\hskip 0.1cm}c@{}}
		\space
            &
		{\huge Input $t_0$}&
		{\huge Tracked $t_0$}&
		{\huge Tracked $t_1$}&
		% {\small Tracked $t_2$}&
		% {\small Tracked $t_3$}\\

   %           \rotatebox[origin=c]{90}{{\large  Similar colored cars}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/26_gt.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/26_bbox.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene1/28_bbox.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}\\[0.95cm]

           \rotatebox[origin=c]{90}{{\Large \textbf{(a)} Shadow}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/21.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene12/22.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
  \\[0.01cm]

            \rotatebox[origin=c]{90}{{\Large \textbf{(b)} Reflection}}&
  		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/gt_img.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/5.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_waymo_results/scene4/6.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
  \\[0.01cm]
  
           \rotatebox[origin=c]{90}{{\Large \textbf{(c)} Occlusion}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene7/0118_4_gt.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene7/0118_4_bbox.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene7/0118_6_bbox.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
   \\[0.01cm]
        
        \rotatebox[origin=c]{90}{{\Large \textbf{(d)} Obstruction}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/rainy_scene/gt_img.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/rainy_scene/30.png}}&
		 \raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/rainy_scene/31.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		 % \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
   \\[0.01cm]

   		\rotatebox[origin=c]{90}{{\Large \textbf{(e)} Det. Accuracy}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene2/2_gt.png}}&
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene2/2)bbix.png}} &
		\raisebox{-0.5\height}{\includegraphics[width=.4\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/additional_nuscenes_results/scene2/3_bbox.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}&
		% \raisebox{-0.5\height}{\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}}
\end{tabular}}
\caption{Examples of failure cases, such as lighting (shadows and reflections) or occluded objects, where the reconstructed object differs significantly from the observed object. These visualizations allow us to understand exactly why our model fails at reconstructing and tracking objects. This also allows us to identify ways the representation model and perception pipeline can be improved to incorporate effects that cause the method to fail.}
	\label{fig:interpretability}
 \end{figure}
% \end{wrapfigure}


==> tables/fig_optimization_no_embedding.tex <==
\begin{figure}[t!]
	\centering
\resizebox{0.9\linewidth}{!}{
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{@{}c@{\hskip 0.05cm}c@{\hskip 0.05cm}c@{}}
		{ Input}&
		{w/o $\mathcal{L}_{embed}$}&
		{w/ $\mathcal{L}_{embed}$}&
	
\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optimization_no_trunc_reg/scene2/gt_img.png}&
\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optimization_no_trunc_reg/scene2/noembed.png}&
\includegraphics[width=.38\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/optimization_no_trunc_reg/scene2/im_w_bbox_rgb_out.png}
\end{tabular}}
\caption{\textbf{Truncation Trick.} From left to right, (i) The input observed image, (ii) results without truncation regularize applied and (iii) results with a truncation regularize applied. For images (ii) and (iii), we also show bounding boxes for each object color-coded by the respective predicted object IDs. As shown here, applying the truncation regularizer helps us achieve more accurate textures and better shapes and colors for the predicted car surface by forcing the optimized embedding to be ``well behaved'', i.e., close to the distribution of latent embeddings seen during the training by our representation model.}
\label{fig:optimization_truncation}
\end{figure}




==> tables/rebuttal_fig_optimization_supplement_no_scehdule.tex <==
\begin{figure}[ht!]
	% \vspace{-12pt}
	 \renewcommand{\arraystretch}{0.4}
	\centering
	\resizebox{1\columnwidth}{!}{%
	\begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
	    {\small (a) Input Frame} & {\small (b) w/ Schedule} & {\small (c) wo/ Schedule} \\
    	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
    	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
    	\includegraphics[width=.31\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png}\\
    	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/gt/82_60_gt_img.png}&
    	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/sched/82_60_shed.png}&
    	\includegraphics[width=.31\columnwidth, trim={22cm 17cm 30cm 18cm},clip]{fig/rebuttal_optimization/no_sched/82_60_no_shed.png}\\
    \end{tabular}}\vspace*{-6pt}
	\caption{\textbf{Effect of Optimization Schedule.} (a) observed image, (b) optimized generations using the proposed schedule (see 3.1 \& 3.3), (c) optimized generations using no schedule.
 % , i.e. such that texture codes, shape codes, rotations, translations, and scales are all simultaneously optimized. The ground truth images are faded to show our rendered objects clearly. 
    % The bottom row shows images zoomed in to clearly show our rendered objects.
    % Our schedule allows for more stable optimization, with rendered objects more closely resembling the observed ones. 
 } 
	\label{fig:opt_rebuttal}
	\vspace{-8pt}
\end{figure}

% \begin{figure}[t!]
%     % \vspace{-12pt}
%     \renewcommand{\arraystretch}{0.4}
%     \centering
%     \resizebox{1\columnwidth}{!}{%
%     \begin{tabular}{@{}c@{\hskip .1cm}c@{\hskip .1cm}c@{\hskip .1cm}c@{}}
%         {\small Input Frame} & {\small Initial Guess} & {\small w/ schedule} & {\small wo/ schedule} \\
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/gt/11_102_gt.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/init_guess/11_102_init.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/sched/11_102_sched.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/rebuttal_optimization/no_sched/11_102_no_sched.png}\\
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}&
%         \includegraphics[width=.23\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{fig/placeholder-img.png}\\
%     \end{tabular}}\vspace*{-6pt}
%     \caption{\textbf{Effect of having an optimization schedule.} From left to right, we show (i) observed image from a single camera, (ii) initial guess, (iii) with schedule, and (iv) without schedule. \todo{describe the figure.}} 
%     \label{fig:opt_supplement}
%     \vspace{-8pt}
% \end{figure}


==> tables/rebuttal_matching_ablations.tex <==
\begin{table}[t!]\label{tab:ablations}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|lll}
\hline
\hline
    Method (split)            & AMOTA $\uparrow$  & Recall $\uparrow$ & MOTA $\uparrow$   \\
    \hline
    AB3DMOT + CP (test) & 0.387             & 0.506             & 0.284             \\
    \hline
    Best Hyper-parameters (test)       & \textbf{0.402}    & \textbf{0.511}    & \textbf{0.320        }     \\
    \hline
    $w_{iou} = 1.4 $ (validation)   & 0.403             & 0.540             & 0.322               \\
    $w_{center} = 0.9$ (validation) & 0.417             & 0.514             & 0.332             \\
    $w_{embedd} = 0.4$ (validation) & 0.418             & 0.558             & 0.332             \\
    $\tau_{det} = 0.4$ (validation) & 0.397             & 0.567            & 0.326             \\
\hline
\hline
\end{tabular}
}
\caption{\textbf{Optimized Matching and Detection Confidence.} Parameters were optimized on the nuScenes \cite{caesar2020nuscenes} validation set. On the test split our best setting with $w_{iou} = 1.4$, $w_{center} = 0.9$, $w_{embbed} = 0.4$, $\tau_{det} = 0.4$ surpasses the performance of AB3DMOT \cite{weng2020AB3DMOT}, the only baseline not trained on the dataset. Results for other baselines are given in Tab. \ref{tab:nuScenes_results}. }\label{tab:rebuttal_ablations}
\vspace{-12pt}
\end{table}

% 1. AB3DMOT
% 2. $w_{iou} = ...$ ..., ...
% 3. $w_{center}$
% 4. $w_{embedd}$
% 5. $\tau_{det}$
% 6. Best

 




==> tables/tab_ablate_matching.tex <==
\begin{table}[ht!]
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|lll}
\hline
\hline
    Method (split)            & AMOTA $\uparrow$  & Recall $\uparrow$ & MOTA $\uparrow$   \\
    \hline
    AB3DMOT + CP (test) & 0.387             & 0.506             & 0.284             \\
    \hline
    Best Hyper-parameters (test)       & \textbf{0.402}    & \textbf{0.511}    & \textbf{0.320        }     \\
    \hline
    $w_{iou} = 1.4 $ (validation)   & 0.403             & 0.540             & 0.322               \\
    $w_{center} = 0.9$ (validation) & 0.417             & 0.514             & 0.332             \\
    $w_{embedd} = 0.4$ (validation) & 0.418             & 0.558             & 0.332             \\
    $\tau_{det} = 0.4$ (validation) & 0.397             & 0.567            & 0.326             \\
\hline
\hline
\end{tabular}
}
\caption{\textbf{Optimized Matching and Detection Confidence.} Parameters were optimized on the nuScenes \cite{caesar2020nuscenes} validation set. On the test split our best setting with $w_{iou} = 1.4$, $w_{center} = 0.9$, $w_{embbed} = 0.4$, $\tau_{det} = 0.4$ surpasses the performance of AB3DMOT \cite{weng2020AB3DMOT}, the only baseline not trained on the dataset. Results for other baselines are given in Tab. \ref{tab:nuScenes_results}. \todo{rewrite} }\label{tab:matching_ablations}
\vspace{-12pt}
\end{table}

==> tables/tab_ablate_optim.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|lll}
    \hline
    \hline
    Method & AMOTA $\uparrow$ & Recall $\uparrow$  & MOTA$\uparrow$  \\
    \hline
    No Schedule & 0.102 & 0.224 & 0.110  \\
    \hline
    $\mathcal{L}_{RGB}$ - Eq.~\ref{eq:loss_mse} & N/A  & N/A & N/A  \\
    $\mathcal{L}_{perceptual}$ - Eq.~\ref{eq:loss_lpips} & 0.100 & 0.251 & 0.101 \\
    $\mathcal{L}_{IR}$ - Eq.\ref{eq:loss_mse_lpips}  & 0.103 & 0.236   & 0.112 \\
    $\mathcal{L}_{IR}$ \& $\mathcal{L}_{embed}$ - Eq.\ref{eq:regularize}  & \textbf{0.112} & \textbf{0.264 } & \textbf{0.113} \\
\hline
\hline
\end{tabular}
}
\caption{\todo{(a) Make split figure} \textbf{Ablation Experiments on Optimization Schedule and Loss Components.} Ablations were run on a small subset of the nuScenes~\cite{caesar2020nuscenes} validation set.  $\mathcal{L}_{RGB}$ fails due to the optimizer fitting objects to the background instead, increasing the size of each object resulting in out of memory.}
\label{tab:optim_ablations}
\end{table}

